ExoClock Project III: 450 new exoplanet ephemerides from ground and space observations

The ExoClock project has been created with the aim of increasing the efficiency of the Ariel mission. It will achieve this by continuously monitoring and updating the ephemerides of Ariel candidates over an extended period, in order to produce a consistent catalogue of reliable and precise ephemerides. This work presents a homogenous catalogue of updated ephemerides for 450 planets, generated by the integration of $\sim$18000 data points from multiple sources. These sources include observations from ground-based telescopes (ExoClock network and ETD), mid-time values from the literature and light-curves from space telescopes (Kepler/K2 and TESS). With all the above, we manage to collect observations for half of the post-discovery years (median), with data that have a median uncertainty less than one minute. In comparison with literature, the ephemerides generated by the project are more precise and less biased. More than 40\% of the initial literature ephemerides had to be updated to reach the goals of the project, as they were either of low precision or drifting. Moreover, the integrated approach of the project enables both the monitoring of the majority of the Ariel candidates (95\%), and also the identification of missing data. The dedicated ExoClock network effectively supports this task by contributing additional observations when a gap in the data is identified. These results highlight the need for continuous monitoring to increase the observing coverage of the candidate planets. Finally, the extended observing coverage of planets allows us to detect trends (TTVs - Transit Timing Variations) for a sample of 19 planets. All products, data, and codes used in this work are open and accessible to the wider scientific community.

==> tab_private_observatories.tex <==

Adrian  Jones & I64, Maidenhead, UK \\
Leon  Bewersdorff & Observatory Kipshoven, Germany \\
Richard  Abraham & The Green Observatory, UK \\
Vikrant Kumar Agnihotri & Cepheid Observatory, Rawatbhata, India \\
Raniero  Albanesi & 157FrassoSabino \\
Enrique Arce Mansego & Vallbona Observatory Valencia España \\
Matthieu  Bachschmidt & Gonachon, France \\
David  Bennett & Rickford Observatory \\
Paul  Benni & Acton Sky Portal, Acton, MA, USA \\
Patrick  Brandebourg & Observatoire du Guernet, Bretagne, France \\
Stephen M. Brincat & Flarestar Observatory (MPC:171), San Gwann, Malta \\
Sebastien  Brouillard & Observatoire de Saint-Véran - Paul Felenbok - France \\
Mauro  Caló & Cavallino Observatory, Tuscany, Italy \\
Fran  Campos & Puig d'Agulles Observatory (Vallirana, Spain) \\
Roland  Casali & Alto2000 Observatory, Italy \\
Giovanni Battista  Casalnuovo & Filzi School Observatory (Laives - Italy) \\
Matteo  Cataneo & Osservatorio Astronomico Civico "G. Barletta", Italy \\
Giuseppe  Conzo & Explorer Orbanic Observatory, Croatia \\
Mercedes  Correa & Sirius B (Spain) \\
Martin Valentine Crow & Burnham Observatory, Burnham on Crouch, UK \\
Dominique  Daniel & LMJ-OBS - private observatory - France \\
Marc  Deldem & Les Barres Observatory, Lamanon, France \\
Dimitrios  Deligeorgopoulos & Artemis Observatory, Evrytania, Greece \\
Salomon Louw Ferreira & PESCOPE \\
Alvaro Fornas Silva & Centro Astronómico Alto Turia (CAAT) \\
Davide Gabellini & Hypatia Observatory, Italy \\
Trevor  Gainey & Kismet observatory, Berkshire, UK \\
Alberto  García-Sánchez & Observatorio Rio Cofio - Robledo de Chavela (Spain) \\
Rafael González Farfán & Uraniborg Observatory, (Écija, Sevilla, Spain) \\
Ferran  Grau Horta & Observatori de Ca l'Ou, Sant Martí Sesgueioles, Spain \\
Tim  Haymes & Tim Haymes Southside Observatory, N.Oxfordshire, UK \\
Francois  Hurter & Albireo Observatory, Switzerland \\
Kevin  Johnson & Holbrook Observatory, East Sussex, UK \\
Aziz Kaeouach Ettahar & High Atlas Observatory, Oukaimeden, Morocco \\
Didier  Laloum & Observatoire Privé du Mont 40280 Saint-Pierre-du-Mont, France \\
Thomas  Mollier & Tomastro Observatory, France \\
Massimiliano  Mannucci & Osservatorio Astronomico Margherita Hack, Firenze, Italy \\
Antonio  Marino & Telescopio Remoto Colacevich c/o Osservatorio Astronomico di Capodimonte di Napoli \\
Giuseppe  Marino & Osservatorio GAC "Luigi Sturzo", Italy \\
Nico Montigiani & Osservatorio Astronomico Margherita Hack, Firenze, Italy \\
Fernando Antonio Martínez & Chile \\
Paolo Arcangelo  Matassa & P.M.P.H.R. Deep Sky (MPC K81) Atina (FR) Italy \\
Philip  Michel & Verulamium Private Observatory, St Albans, UK \\
Mike  Miller & Georgetown Observatory, Georgetown, TX USA \\
Mario  Morales-Aimar & Observatorio de Sencelles, Spain \\
Fabio  Mortari & Hypatia Observatory, Italy \\
Jean-Louis  Naudin & Gatinais French Observatory (GFO) \\
Zlatko  Orbanic & Explorer \\
Christian  Pantacchini & Observatoire de BENAYES ; FRANCE \\
Jean-Bernard  Pioppa & La Roque Esclapon - FRANCE \\
Nikolaos I. Paschalis & Nunki Observatory, Skiathos, Greece \\
Valère  Perroud & Observatoire de Duines, France \\
Mark  Phillips & Forthimage Observatory, Edinburgh, Scotland \\
Jeff  Purcell & Omaha, Nebraska-United States \\
Manfred  Raetz & Privat Observatory Herges-Hallenberg, Germany \\
François  Regembal & HRT Observatory, Spain \\
Lionel  Rousselot & Vierzon Observatory, France \\
Xesco  Rubia & Stupa Observatori, Centelles, Catalonia, Spain \\
Nello  Ruocco & Osservatorio Astronomico Nastro Verde, Sorrento, Italy \\
Mark  Salisbury & POST, UK \\
Fabio  Salvaggio & WBRO (K49), Italy \\
John  Savage & Z42, Rushay Farm Observatory, Dorset, UK \\
Danilo  Sedita & Osservatorio Sedita Castrofilippo, Italy \\
Nick  Sioulas & NOAK Observatory L02, Greece \\
Dimitris  Stouraitis & Galileo Observatory, Greece \\
Geoffrey  Thurston & I67, Hartley Wintney, UK \\
Andrea  Tomacelli & Telescopio Remoto Colacevich UAN c/o Osservatorio Astronomico di Capodimonte di Napoli \\
Alberto  Tomatis & Alto-Observatory, Italy \\
Pierre  Valeau & Observatoire de l’Aiguillon sur Mer, France \\
Jean-Pascal  Vignes & Deep Sky Chile , Chile \\
Kuldip  Vora & Cepheid Observatory, Rawatbhata, India \\
David E. Wright & Yorick Observatory, Hampshire, UK \\
Vojtěch  Školník & Broumov NM Observatory, Czech Republic \\


